NetBench: A Large-Scale and Comprehensive Network Traffic Benchmark Dataset for Foundation Models

In computer networking, network traffic refers to the amount of data transmitted in the form of packets between internetworked computers or Cyber-Physical Systems. Monitoring and analyzing network traffic is crucial for ensuring the performance, security, and reliability of a network. However, a significant challenge in network traffic analysis is to process diverse data packets including both ciphertext and plaintext. While many methods have been adopted to analyze network traffic, they often rely on different datasets for performance evaluation. This inconsistency results in substantial manual data processing efforts and unfair comparisons. Moreover, some data processing methods may cause data leakage due to improper separation of training and testing data. To address these issues, we introduce the NetBench, a large-scale and comprehensive benchmark dataset for assessing machine learning models, especially foundation models, in both network traffic classification and generation tasks. NetBench is built upon seven publicly available datasets and encompasses a broad spectrum of 20 tasks, including 15 classification tasks and 5 generation tasks. Furthermore, we evaluate eight State-Of-The-Art (SOTA) classification models (including two foundation models) and two generative models using our benchmark. The results show that foundation models significantly outperform the traditional deep learning methods in traffic classification. We believe NetBench will facilitate fair comparisons among various approaches and advance the development of foundation models for network traffic. Our benchmark is available at https://github.com/WM-JayLab/NetBench.

==> back.terms.tex <==
Data that is in-distribution can be called novelty data 


The term 'out-of-distribution' (OOD) data refers to data that was collected at a different time, and possibly under different conditions or in a different environment



==> secs/preliminary.tex <==
% \section{Preliminaries} \label{sec:preliminary}
% In this section, we first present the problem of detecting OOD samples for data of multiple modalities and then review contrastive learning for multi-modal OOD detection.


% \subsection{Problem Statement}
% We consider the problem of detecting multi-modal OOD samples under three different scenarios, as mentioned in Section~\ref{sec:intro}. In this paper, we use vision-language modeling as a running problem for multi-modal OOD detection. With a batch of $N$ pairs of images and texts, along with their labels, denoted by $\{(x_n, t_n), y_n\}_{n=1}^N$, there is a very small number of samples, $K$, that are OOD in the three scenarios above and the remaining $N-K$ pairs are ID samples. The goal of this work is to distinguish the OOD samples from the ID ones using weakly-supervised learning.


% \subsection{Contrastive Representation Learning}
% Contrastive representation learning aims to encode pairs of data samples into latent representations by making similar samples close to each other and dissimilar ones far apart. One well-known method is the vision-language pre-trained model CLIP, which jointly trains an image encoder and a text encoder to learn the latent representations from text paired with images using zero-shot learning. Specifically, it encodes a pair of image $x_n$ and text $t_n$ into the latent representations $\mathcal{I}(x_n) $ and $\mathcal{T}(t_n)$, respectively, and then adopts cosine similarity to minimize the distance of their representations $\mathcal{I}(x_n)$ and $\mathcal{T}(t_n)$. Due to its excellent performance in learning the latent representations of images and texts, a few CLIP-based methods have been developed to detect multi-modal OOD samples. However, existing methods can only detect one specific scenario where a given image and its textual information come from a new domain with a distribution shift. In the following section, we develop a general-purpose OOD detection framework to identify OODs arising from several different scenarios.

